Differentially Private Call Auctions and Market Impact

We propose and analyze differentially private (DP) mechanisms for call auctions as an alternative to the complex and ad-hoc privacy efforts that are common in modern electronic markets. We prove that the number of shares cleared in the DP mechanisms compares favorably to the non-private optimal and provide a matching lower bound. We analyze the incentive properties of our mechanisms and their behavior under natural no-regret learning dynamics by market participants. We include simulation results and connections to the finance literature on market impact.

==> meta_algo.tex <==

%We provide a meta algorithm that simply computes the difference of  payoff bounds of Mechanisms~\ref{alg:mech} and~\ref{alg:mech_lottery}
We do so by computing the difference of payoff bounds of Mechanisms~\ref{alg:mech} and~\ref{alg:mech_lottery}
$$
f \triangleq \frac{2 \ln \left( 1/\alpha \right)}{\epsilon}  + \sqrt{ 6  \left(\opt + \frac{\ln (1/\alpha)}{\epsilon} \right) \ln \left(1/\alpha\right)} - \frac{4 \ln (n/ \alpha)}{\epsilon}
$$
in a differentially privately manner.\footnote{$\opt$ is a function of the input data set, hence a direct comparison of the bounds without addition of noise may leak information about the reported bids.} Then, based on the sign of $f$, the mechanism decides whether to run $\M_1$ or $\M_2$. The private computation of $f$ will unavoidably add an extra term of order $\bigo (1/\epsilon)$ to the payoff bound.

\begin{algorithm}
    \SetAlgoNoLine
	\KwIn{Agents' valuations $(\vs,\vb)$, privacy level $\epsilon$, confidence level $\alpha$.}
    \KwOut{Market price $p$, allocations $\oo=(\os,\ob)$.}
	$f \gets \frac{2 \ln \left( 1/\alpha \right)}{\epsilon}  + \sqrt{ 6  \left(\opt + \frac{\ln (1/\alpha)}{\epsilon} \right) \ln \left(1/\alpha\right)} - \frac{4 \ln (n/ \alpha)}{\epsilon}$
	
	$\widetilde{f} \gets f + Lap \left(\frac{\sqrt{6 \ln(1/\alpha)}}{\epsilon} \right)$ \Comment{Private estimate of $f$}
	
	\eIf{$\widetilde{f} < 0$}
	{
		Run $\M_1 \left(\vs,\vb,\epsilon, \alpha \right)$ (Algorithm \ref{alg:mech}) and get $p,\oo$.
    }
    {
		Run $\M_2 \left(\vs,\vb,\epsilon \right)$ (Algorithm \ref{alg:mech_lottery}) and get $p,\oo$.
	}
	\caption{Private Call Auction with Allocation: A Meta Algorithm ($\M_3$)}
	\label{alg:mech_combined}
\end{algorithm}


\begin{clm}[Joint DP]\label{clm:DP_3}
	The allocation mechanism described in Algorithm \ref{alg:mech_combined} is $7\epsilon$-joint DP.
\end{clm}

\begin{thm}[Payoff and Inventory of Mechanism]\label{thm:thm_3}
Suppose $\opt \geq 5 \ln (V/\alpha)/\epsilon$.
\begin{enumerate}
\item Payoff: with probability $1-18\alpha$,
\begin{align*}
&\Pi \left( \M_3 \right)  \\
&\ge \opt - \frac{2 \ln (\frac{V}{\alpha})}{\epsilon} - \min\left\{ \frac{2 \ln \left( \frac{1}{\alpha} \right)}{\epsilon}  + \sqrt{ 6  \left(\opt + \frac{\ln (\frac{1}{\alpha})}{\epsilon} \right) \ln \left(\frac{1}{\alpha}\right)},  \frac{4 \ln (\frac{n}{\alpha})}{\epsilon} \right\} - \frac{\sqrt{6} \ln^{1.5} (\frac{1}{\alpha})}{\epsilon}
\end{align*}

\item Inventory: with probability $1-14\alpha$,
\begin{align*}
&I \left( \M_3 \right) \\
&\le 4 \min\left\{ \frac{2 \ln \left(\frac{1}{\alpha} \right)}{\epsilon}  + \sqrt{ 6  \left(\opt + \frac{\ln \left(\frac{1}{\alpha}\right)}{\epsilon} \right) \ln \left(\frac{1}{\alpha}\right)},  \frac{4 \ln (\frac{n}{\alpha})}{\epsilon} \right\} +  \frac{4 \sqrt{6} \ln^{1.5} (\frac{1}{\alpha})}{\epsilon} + \frac{10 \ln (\frac{1}{\alpha})}{\epsilon} + \frac{4 \ln (\frac{2}{\alpha})}{3}
\end{align*}

\end{enumerate}
\end{thm}

This theorem follows from Theorems \ref{thm:thm_1} and \ref{thm:thm_2}, as well as the accuracy guarantee of the Laplace mechanism used in Algorithm \ref{alg:mech_combined} to compute $f$. We defer the full proof to Appendix~\ref{app:mechanism3}.
